iFixR: Bug Report driven Program Repair

Issue tracking systems are commonly used in modern software development for collecting feedback from users and developers. An ultimate automation target of software maintenance is then the systematization of patch generation for user-reported bugs. Although this ambition is aligned with the momentum of automated program repair, the literature has, so far, mostly focused on generate-and-validate setups where fault localization and patch generation are driven by a well-defined test suite. On the one hand, however, the common (yet strong) assumption on the existence of relevant test cases does not hold in practice for most development settings: many bugs are reported without the available test suite being able to reveal them. On the other hand, for many projects, the number of bug reports generally outstrips the resources available to triage them. Towards increasing the adoption of patch generation tools by practitioners, we investigate a new repair pipeline, iFixR, driven by bug reports: (1) bug reports are fed to an IR-based fault localizer; (2) patches are generated from fix patterns and validated via regression testing; (3) a prioritized list of generated patches is proposed to developers. We evaluate iFixR on the Defects4J dataset, which we enriched (i.e., faults are linked to bug reports) and carefully-reorganized (i.e., the timeline of test-cases is naturally split). iFixR generates genuine/plausible patches for 21/44 Defects4J faults with its IR-based fault localizer. iFixR accurately places a genuine/plausible patch among its top-5 recommendation for 8/13 of these faults (without using future test cases in generation-and-validation).

==> oldabstract.tex <==
%Most open source projects include an open issue tracker (e.g, Bugzilla, Jira) system to engage users in  development and testing activities as well, discussion of potential enhancements, reporting issues and validation of the patches. Although automated program repair holds the promise of reducing the manual debugging efforts through automatically generating patches, it is not yet adopted by the open source practitioners.
%The unrealistic setup of the APR tools is one the main reasons for the lack of adoption. The current practices rely on future data (i.e., the information that is not available when the bug has been reported) both for localizing the bugs and as the oracle for validating the generated patches. With this study, we present Mimic, a new pipeline for APR, which imitiates the fundamental steps in a real bug fixing lifecycle to overcome the biases due to the usage of future data. Concretely, we focus on (a) bug reports to identify the suspicious buggy code localization (b) patch validation without using future test cases.


% In a typical APR pipeline, given a buggy program, a fault localization tool is leveraged to identify the suspicious buggy code locations using passing and failing test cases in a manually curated benchmark. 


% Defect4J, is a widely used benchmark for APR studies where 357 bugs from open source programs with test cases are reproduced in an isolated manner. However, none of the APR tools consider whether test cases are available when the bug inducing commit has been made. In a realistic setup, the fault localization could be performed only with the information available when the bug has been reported. We perform an empirical study on Defect4J benchmark to verify the existence of the test cases at the moment the bug inducing commit has been made.
% The initial results suggest that only 14 bugs of Defect4J them have failing test cases before the developer bug fixing patch is applied. The remaining test cases (96\% of Defect4J bugs) are either inserted or modified with developers bug fixing patch. 

% This finding implies current APR pipelines cannot be applied in a realistic setup since the current practices rely on future test cases to identify the suspicious buggy code locations. We propose a novel approach that mimics the steps of developer during the bug fixing process in open source projects. 

% We start by collecting bug fixing patches from 45 java projects with their corresponding bug reports and apply D\&C


% In a realistic setup, bug fixing is done as follows. First, when an unexpected behavior is monitored a project, a bug report is filed, describing the failure. Then, the bug report is verified by the maintainers and assigned to a developer if the bug is verified.
% To fix the bug, the developer clones the project repository, replicates the bug, locates the buggy code.  Finally, the developer proposed a patch, most likely with test cases covering the buggy code.




==> tables/flResultDC.tex <==
\begin{table}[!h]
	\centering
	\scriptsize
	\caption{Fault localization results of D\&C}%(171 bugs)
	\begin{threeparttable}
		\begin{tabular}{c|c|c|c|c|c}
			\toprule
			Top-1 & Top-10 & Top-50 & Top-100 & Top-200 & All
			\\\cline{0-5}
			55 & 131 & 147 & 151 & 153 & 154 \\
			\bottomrule
		\end{tabular}

	\end{threeparttable}
	\label{tab:flresultsDC}
\end{table}
